SpaBERT: A Pretrained Language Model from Geographic Data for Geo-Entity Representation

Named geographic entities (geo-entities for short) are the building blocks of many geographic datasets. Characterizing geo-entities is integral to various application domains, such as geo-intelligence and map comprehension, while a key challenge is to capture the spatial-varying context of an entity. We hypothesize that we shall know the characteristics of a geo-entity by its surrounding entities, similar to knowing word meanings by their linguistic context. Accordingly, we propose a novel spatial language model, SpaBERT, which provides a general-purpose geo-entity representation based on neighboring entities in geospatial data. SpaBERT extends BERT to capture linearized spatial context, while incorporating a spatial coordinate embedding mechanism to preserve spatial relations of entities in the 2-dimensional space. SpaBERT is pretrained with masked language modeling and masked entity prediction tasks to learn spatial dependencies. We apply SpaBERT to two downstream tasks: geo-entity typing and geo-entity linking. Compared with the existing language models that do not use spatial context, SpaBERT shows significant performance improvement on both tasks. We also analyze the entity representation from SpaBERT in various settings and the effect of spatial coordinate embedding.

==> note.tex <==
%Place names can be quite ambiguous without the spatial context. In the sentence "My trip to the Springfield was wonderful", you might wonder which Springfield that it is referring to, as there are hundreds of Springfields within the US. But if we say "My trip to the Springfield was wonderful, we also took a walk along the Connecticut River", then we know that it is the Springfield in Massachusetts. So what makes a place different from others? Although this is an open question, but from the example above, we can see that the spatial context (i.e. other nearby geo-entities) plays an important role in representing a place. 
% not dealing with sentences. 


% Hence they are widely used for organizing geo-spatial information not only for traffic and tourism, but also in studies for urban planning an geography \textcolor{red}{[citation]}. 

%To distill the information and extract features for the geo-entities within the map, machine learning models need to handle the composite of various concepts (e.g. text, symbols and layout). 

%graphical form to represent the location and spatial relations for various geo-entities. 

%Vast amount of maps are available in libraries and archives, machines can harvest valuable information from maps to assist cultural, economical and anthropological studies. 

%So it is natural to employ Language Models (LMs) to extract informative features for geo-entities. 


 %(1) using map data to enrich the data for document grounding, \textcolor{red}{[citation]} question answering related to maps\textcolor{red}{[citation]} (3) information extraction
 
%The use of maps can be dated back to the 6th Century BCE \textcolor{red}{[citation]}, where the Babylonians carved down the world on clay tablets. Although it is not accurate compared with contemporary ones, it still reflects ancient Babylonians' comprehension of the world. Ever since then, people have continued using maps as a graphical form to convey knowledge and inherits culture. As the maps have been accumulated in the past thousand of years, it is a non-trivial task to analyze the map sheets, and establishing the correspondence between the past and current world. Also for the places that were abandoned, structures that were demolished, we might be able to find some clues in historical maps on what those places were build for. 



 %Understanding and extracting features for the geo-entities contained in the map can be useful for geo-coding, entity linking and geo-tagging \textcolor{red}{[citation]}.

%why ML models need to understand map

%The simplest way to represent the geo-entity is to extract linguistic features using pretrained language models (LMs) such as  FastText or BERT\textcolor{red}{[citation]} given the placename as the input. 


%ViT \textcolor{red}{[citation]} is an attempt to capture 2D context in vision problems by dividing the input image into grids, and further linearize the input to feed into LMs. But this approach has its limitation on maps as maps can be sensitive to the grid size.  Also there might be several geo-entities contained in one grid, LMs would assume the same 2D context for all the geo-entities in the same grid, which is not true in the real world. 


\begin{comment}
\begin{itemize}
  \item Understanding geo-entities requires resolving type and ambiguity which requires spatial context, not only linguistic context. Same location name, different type.  + ramp example.    
  \item  LM uses linear context, not spatial context. Map requires spatial context. 1D v.s. 2D. While pretrained LMs can provide contexual information for lexemes, which can only be applied for linear context. 
  \item In addition, LM pretrained on genneral-purpose domain needs to be fine-tuned on maps to encode spatial information. 
\end{itemize}
\end{comment}


% To be consistent with what this community has been using to represent a multi-token span with a PLM, this should be either average or using the first subtoken representation

%\muhao{How do you get the representation of a pivot entity? how do you use it in specific tasks (classification, linking, etc.). Refer to 2.2 of \url{https://arxiv.org/pdf/2110.08443.pdf} as an example.}

%his is very confusion. there are just two different positional embeddings: the sequential positional embedding is the original one, and there is another spatial position embedding


%`data' is countable and plural


%https://docs.oracle.com/en/cloud/saas/sales/22a/oacdm/overview-of-geographies-geographic-entities-and-locations.html#s20079766

  

\begin{comment}

Challenges for typing:
\begin{itemize}
  \item not able to infer type from name
  \item different types for the same name (find example)
  \item LM trained on newspapers and wikipedia are not suitable for encoding place names. Needs fine-tuning.
\end{itemize}


Challenges for linking:
\begin{itemize}
  \item places with same name
  \item un-georeferenced maps do not have geo-coordinates. 
  \item even with name and location, the location might not be precise (mountain, lake)
  \item granularity on two sides might be different
\end{itemize}

BERT\textsubscript{\textit{base}}
BERT\textsubscript{\textit{large}}
BERT\textsubscript{{\fontfamily{qcr}\selectfont Large }}




\newcommand{\tablelinkingablation}{
\begin{table}
\centering
\resizebox{0.9\columnwidth}{!}{
%\small
%\setlength\tabcolsep{2pt}
\begin{tabular}{lcccc}
\hline \textbf{Model} & \textbf{MRR} & \textbf{R@1} &  \textbf{R@5} & \textbf{R@10} \\ \hline
\modelnamens\modelsub{Base}  &  & & \\
\hspace{1em} - no coord embed & & & \\
\modelnamens\modelsub{Large}  & & & \\
\hspace{1em} - no coord embed  & & & \\
\hline
\end{tabular}
}
\caption{\label{tab:linkingablation} With and without using spatial coordinate embedding }
\end{table}
}

\footnote{If the $g^{loc}$ is in the image coordinate system, then the distance metric is Euclidean distance. If $g^{loc}$ is in the geo-coordinate system, then the distance metric is Haversine distance in kilometers which measures the distance on a sphere.}
\end{comment}



%\modelname, extends the pretrained BERT architecture to enable meaningful encoding of a geo-entity given other geo-entities in its local neighborhood (i.e., the spatial context). Since geo-entity coordinates are 2-dimensional, and existing LMs accepts sequential inputs. Thus to capture the spatial context, we propose a novel approach to linearize geo-entities and their neighboring entities in the 2-dimensional geographical space. The linearized representation preserves the corresponding distance and orientation of geo-entities, and 
%it enables BERT and other language models that expect 1D input (i.e., sentences) to learn spatial context-aware encoding.

%Encoding the meaning of geo-entities (e.g., points of interest) can enable many useful downstream tasks. However, directly encoding their location, name, and type does not fully capture the spatial-varying context of a geo-entity. We hypothesize that we shall know a spatial thing by the company it keeps in the geographical space, similar to knowing a word by its surrounding words. We propose a novel yet simple approach to linearize geo-entities and their neighboring entities in the 2-dimensional geographical space while preserving their corresponding spatial relationship. Our proposed model, \modelname, builds on the pretrained BERT architecture, embeddings does not fully capture the spatial-varying context of a geo-entity. We hypothesize that we shall know a spatial thing by the company it keeps in the geographical space, similar to knowing a word by its surrounding words. Our proposed model, \modelname, builds on the pretrained BERT architecture to enable meaningful encoding of a geo-entity given other geo-entities in its local neighborhood (i.e., the spatial context). Since geo-entity coordinates are 2-dimensional, and existing language models accept sequential inputs. Thus to capture the spatial context, we propose a novel approach to linearize geo-entities and their neighboring entities in the 2-dimensional geographical space. The linearized representation preserves the corresponding distance and orientation of geo-entities, and 
%enabling  BERT and other language models that expect 1D input (i.e., sentences) to learn spatial context-aware encoding. We apply the model to two downstream tasks: geo-entity typing and geo-entity linking. For the geo-entity typing task, we predict the type of geo-entities with a multi-class classification model. For geo-entity linking, we link the entities on maps to the structured knowledge base (e.g., WikiData). Compared with the existing language models that do not utilize spatial context, \modelname shows noticeable performance improvement on both tasks. 


% 1. Arguments that need to be covered in the first paragraph:
% - Maps are an important way of organizing geographical information
% - Machine intelligence needs to understand map information, inasmuch as humans do...
% - Text is the building block of maps, therefore map understanding is dependent on understanding textual information in maps.

%\muhao{This paragraph needs to convince peer reviewers (PR) on 1. machine needs to comprehend maps (support this claim with concrete applications, e.g. QA on maps, IE from maps, information intergration to maps); 2. Natural language text is the building block of map, hence understanding maps requires the machine to understand their textual components.}

%Geographic datasets, such as points of interest (POI) data, contain information about named geographic entities and their locations. There are various existing geographic datasets to encompass contemporary and historical geo-entities, such as OpenStreetMap \cite{osm} as vector data and USGS Historical Topographic Maps Collection\cite{usgs}  as raster images. 

%Named geographic entities (geo-entities) exist in many geographic datasets, such as points of interest (POI) data in OpenStreetMap~\cite{osm} or GeoNames~\cite{} and scanned historical maps (e.g., the United States Geological Survey Historical Topographic Map Collection~\cite{usgs}). The vast amount of named geo-entities in these datasets requires effective comprehension and knowledge discovery technologies to ease the use of this resource in various traffic \cite{liang2017inferring, jiang2018geospatial}, urban design \cite{san2014urban}, economical and anthropological applications \cite{petit2002impact, chiang2020using}. Since the geo-entity name is one of the important attributes in the geographic datasets, machine comprehension of geographic datasets naturally depends on the understanding of the textual information. An effective language model (LM) is therefore needed not only for the purpose of extracting informative features for geo-textual components, but also seek to benefit various tasks such as geo-entity typing and linking. 

%QA on maps, information extraction from maps, as well as geo-entity grounding for maps.



% \muhao{``geo-entity feature representation'' seems to be a bit limited usage of an LM, in comparison to what has been used to motivate the study in the previous paragraph.} 
%Recently, the research community has seen a rapid advancement in pretrained language models (LMs) \cite{devlin-etal-2019-bert,liu2019roberta, lewis2019bart, sanh2019distilbert}, which have supported strong language representation abilities \cite{lan2019albert} and served as the backbones of various NLP systems  \cite{rothe2020leveraging, yang-etal-2019-exploring-pre}. 
%(e.g., for information extraction, entity linking, and semantic parsing).
%However, existing LM methods are still short of capturing spatial relations and structural inputs due to several challenges. First of all, it ignores the relations between geo-entities. The neighboring entities (\textit{spatial context}) are highly correlated with the center geo-entity, and they can potentially provide information on distinguishing two geo-entities of the same name. Thus understanding geo-entities requires parsing the spatial context. Moreover, context-aware LMs are designed to capture 1-dimensional linguistic context in sentences, while geo-coordinate is a 2-dimensional representation. So the spatial context embedding is not supported by the existing model structures. In addition, LMs pretrained on general-purpose domain \cite{devlin-etal-2019-bert,liu2019roberta} needs to be fine-tuned on geographic datasets to encode geographical information. 



%To tackle these challenges, we present \modelname, a language model that captures the spatially varying context of geo-entity names using large geographic datasets for entity representation. Built upon BERT \cite{devlin-etal-2019-bert}, \modelname generates the contextualized representation for a geo-entity of interest (referred to as \textit{pivot}), based on its geographically nearby geo-entities. Specifically, \modelname linearizes the spatial context by forming \textit{pseudo sentences} that consist of names of the pivot and neighboring geo-entities. It also models the relative spatial distance between the pivot and neighboring geo-entities with a continuous \emph{spatial coordinate embedding}. The embedding is composed of two parts: horizontal and vertical embedding. With these techniques, the transformed geo-entity input could be compatible with the BERT-family structures. Since the language models are trained on the general-purpose corpus, they have the domain shift problem when directly applied to the map data. We thus pretrain the model with the linearized spatial context on large-scale geographic datasets derived from the OpenStreetMaps (OSM). The pretraining contains two parts: Masked Language Modeling (MLM) and Masked Entity Modeling (MEM). The MLM randomly masks out the subtokens in the pseudo sentence, and MEP masks out the full location phrase. MLM and MEP enable the \modelname to handle the pseudo sentence input and to learn the relations of geo-entities. 

%Thus the pivot representation is sensitive to the spatial context that it falls within. In the \textit{Ash Wood} example mentioned above, the Ash Wood for forest and the Ash Wood for suburb should be different. 

%For example, the representation of \textit{The Swan} around mountains should be different from that around restaurants, as the former is likely to be a mountain while the later is not. 

%\modelname can be treated as a general-purpose encoder that captures the name and spatial context of geo-entities. 

%en: still not broad enough. broad means: "machine reading comprehension, narrative understanding" those are called broad, "story ending prediction" is not. also, what's special about entity grounding?

%\muhao{A central question to this abstract: currently there isn't any description about what data modality the model works on.}
%Named geo-entities (e.g., points of interest) 

%such as OpenStreetMap and GeoNames. %A named geo-entity contains two major components: its name and geo-location (e.g., point or polygon geo-coordinates), which can be used for entity grounding and other applications. 

%However, directly encoding their names and locations does not fully capture the spatial-varying context of a geo-entity. 

%We propose a novel approach to linearize geo-entities and their neighboring entities in the 2-dimensional geographical space while preserving their corresponding spatial relationship. 

%why is this related to a map? Most NLP people does not even know what a spatial database is FY

 % we need to put at least a footnote to say a spatial database stores all entries in the map or other types of repository we seek to represen
 
 %domain-specific means things like BioBERT, Clinical BioBERT, SciFive, BERTOverflow, etc.
 
 %You can just introduce there are a couple of LMs dedicated to this domain, including A B C. They are typically adapted to this domain in this way, and typically address tasks X, Y, Z. Then in another domain (same). However we are the first attempt in Zekun domain.

==> s2-6234pm.tex <==
\section{\modelname}

We first describe the overall architecture in \Cref{sec:overall} and then show how \modelname represents geo-entities in \Cref{sec:spatial_context}, followed by the pretraining and inference procedure in \Cref{sec:pretrain} and \Cref{sec:inference}. 


%\muhao{refer to
%\url{https://arxiv.org/pdf/2110.08443.pdf} + TaBERT and Tapas papers when writing this section.}

\begin{figure*}[t]
  \begin{center}
	\includegraphics[width=1.0\linewidth]{figures/embedding1.png}
  \end{center}
  \caption{Spatial context encoding. Input to the token-embedding is the tokenized pseudo-sentence. Input to the position embedding is the index of the token. Input to the spatial coordinate embedding embedding are the normalized distances from pivot (details in \Cref{sec:spatial_context}). }
  \label{fig:sbert_embedding}
\end{figure*}



\subsection{Preliminary}\label{sec:overall}

% preliminary: define input only. -> move SC related part to 2.2.1
% what is spatial context of the map and how to linearize it. 
% based on BERT, what is spatial context representation. 2-dimensional-? linear context, added spatial embedding to encode position information. design mlM,mem for pretraining,  support xxx inference tasks, the following contains details of each component. 


% \muhao{define your data (abstract with notations), and describe the overall architecture/workflow/components of your model.}


\modelname is a LM built upon a pretrained BERT model and further trained to produce contextualized representations of geo-entities given large geographic datasets. \Cref{fig:sbert_outline} shows the overview of the proposed method.
The spatial context is the surrounding area near the pivot entity, which contains 
neighboring geo-entities.
The range of the context can be bounded based on the distance from the pivot or an upper limit of the number of neighboring entities.
To convert the 2-dimensional spatial context to sequential input
that is compatible with the BERT structure, \modelname linearize the neighboring geo-entities into distance-ordered entity sequences called \emph{psuedo-sentences}. 
To capture the location information of the entities, in addition to the original (sequential) positional embedding in BERT, we also design a spatial coordinate embedding mechanism. (Details in \Cref{sec:spatial_context})
We optimize \modelname using both the masked language modeling (MLM) and a masked entity prediction (MEP). The resulting model can
support downstream inference tasks such as geo-entity typing and geo-entity linking. Details of the technical components are described in the rest of this section.


\subsection{Spatial Context Representation} \label{sec:spatial_context}



We assume that in the geographic datasets $S = \{g_1, g_2, ..., g_l\}$, each geo-entity $g_i$ is associated with two attributes: name $g^{name}$ and location $g^{loc}$, where $g^{loc}$ is a tuple $g^{loc} = (g^{locx}, g^{locy})$ that identifies the location in a certain coordinate system (e.g. image pixel coordinates or EPSG:4326 geo-coordinates\footnote{More information about EPSG:4326 can be found at: https://epsg.io/4326}). The goal of the \modelname is to extract feature for a geo-entity $g_i$  given the $g^{name}$, $g^{loc}$, and spatial context. The central geo-entity that we %want
seek to %represent
generate a contextualized representation for is referred as the \emph{pivot entity} $g_p$, 
and 
the set of neighboring geo-entities within its spatial context are $SC(g_p) = \{g_{n_1},...,g_{n_k}\}$ where $dist(g_p, g_{n_k}) < T$. For short, we will denote the pivot as $p$ and the neighboring entities as $n_1, ..., n_k$ when there is no confusion. 


\stitle{Constructing Spatial Context}  Given the pivot entity, we first obtain the neighboring entities within the spatial context. Then the neighboring entities are sorted in ascending order based on the distance. The pseudo sentence is formed by concatenating the pivot and neighboring entity names. The pseudo sentence is tokenized with the original BERT tokenizer with separator [SEP] between entities. For the example in \Cref{fig:sbert_outline}, the corresponding pseudo sentence %should be:
is accordingly constructed as:



\begin{center}
\noindent\fbox{%
    \parbox{0.9\linewidth}{%
     {\fontfamily{cmtt}\selectfont
        [CLS] University of Minnesota [SEP] Minneapolis [SEP] St. Anthony Park [SEP] Bloom Island Park [SEP] Bell Museum [SEP] }
    }%
}
\end{center}
Similar to BERT, \modelname calculates the embedding for each input token. To get the pivot entity representation $E^p$, the token level embeddings for the pivot entity $E^p_1, ..., E^p_m$ are averaged to produce a fixed-length vector.



\stitle{Spatial Coordinate Embedding} The token embeddings of pseudo-sentences are incorporated with two types of positional embeddings (See \Cref{fig:sbert_embedding}.
%One is the \emph{original (sequence) position embedding}, same as the one in BERT, represents the indices of tokens in the pseudo-sentence. 
In addition to the original (sequence) position embedding in BERT and other Transformer LMs,
%This embedding preserves the order information of the tokens in the same geo-entity name. 
%The other one is the
\modelname incorporates a \emph{spatial coordinate embedding} mechanism which seeks to represent the relative geo-entity distances from pivot $p$ to a neighbor $n_k$. Since the spatial context is 2D, we divide this coordinate embedding into two parts, one for horizontal direction (x-axis) and the other for vertical direction (y-axis). 
The $dist_x^{n_k}$ and $dist_y^{n_k}$ are the normalized distance input to the spatial coordinate embedding, and they are calculated as:
\begin{align*}\label{eq:dist}
    dist_x^{n_k} = (g_{n_k}^{locx} - g_p^{locx})/Z \\
    dist_y^{n_k} = (g_{n_k}^{locy} - g_p^{locy})/Z
\end{align*}
where ($g_{p}^{locx}$,$g_{p}^{locx}$) is the pivot entity location and ($g_{n_k}^{locx}$,$g_{n_k}^{locx}$) is the neighboring entity location, $Z$ is a normalization factor. Notice that tokens belong to the same geo-entity have the same $dist_x^{n_k}$ and $dist_y^{n_k}$. \texttt{DSEP} is constant numerical value works as the distance separator. It should be larger than $max(g_{n_k}^{locx},g_{n_k}^{locx})$ for all neighboring entities, so as to differentiate the special tokens from the geo-entity name tokens. 


The $dist_x^{n_k}$ and $dist_y^{n_k}$ inputs are encoded with a continuous spatial coordinate embedding layer. Instead of discretizing the input distances to integer values like the position embedding of tokens, we use the real-valued distance directly as the input to preserve the continuity of the output embeddings. 

Let $M$ be the dimension of the embedding features, $\mathcal{S}_{n_k}$ be the spatial coordinate embedding of the entity $n_k$, and $\mathcal{S}_{n_k} \in \mathbf{R}^M$. Then $\mathcal{S}_{n_k}$  can be defined as
\begin{align*}
  \mathcal{S}_{n_k}^{(m)} = 
  \begin{cases}
    sin(dist^{n_k}/10000^{2j/M}), m = 2j  \\
    cos(dist^{n_k}/10000^{2j/M}), m = 2j+1 
  \end{cases}
\end{align*}
where $\mathcal{S}_{n_k}^{(m)}$ is the $m$-th dimension of $\mathcal{S}_{n_k}$, and $dist^{n_k}$ can be substituted by $dist_x^{n_k}$ for the embedding along horizontal direction, and $dist_y^{n_k}$ for the vertical direction.
%\muhao{this part is missing connection to your Spatial-X and Spatial-Y.}


\subsection{Pretraining}\label{sec:pretrain}
We further train the model with two pretraining tasks to adapt the pretrained BERT backbone to the geo-entity data. 
In addition to the masked language modeling (MLM)  \cite{devlin-etal-2019-bert}, 
we also include a masked entity prediction (MEP) task. Both MLM and MEP have a masking rate of 15\%.\footnote{The [CLS] and last [SEP] token are not masked out.} The two pretraining tasks are based on the intuition that the geo-entity location and spatial context should contain information to recover the masked geo-entity. 
In the scenario of representing a spatial context,
MLM randomly masks out some individual subtokens in the pseudo sentence and teaches the \modelname to complete the full name of a geo-entity with the partial name, location, and surrounding geo-entities. The block below shows an example of the masked input for MLM, where \#\#\# are the subtokens that have been masked out:

\begin{center}
\noindent\fbox{%
    \parbox{0.9\linewidth}{%
    {\fontfamily{cmtt}\selectfont
        [CLS] \#\#\#  of Minnesota [SEP] Minneapolis [SEP] St. \#\#\# Park [SEP] \#\#\# Island Park \#\#\# Bell Museum [SEP] }
    }%
}
\end{center}

The MEP is designed to learn entity-level representations and helps capture spatial context information. %MEP first
Hence, MEP randomly chooses an entity in the pseudo-sentence and masks out all the subtokens belonging to that entity. The \modelname needs to rely on the masked entity position and the neighboring entity names and positions to recover the name of the masked entity. The block below shows an example of the MEP input. 

\begin{center}
\noindent\fbox{%
    \parbox{0.9\linewidth}{%
     {\fontfamily{cmtt}\selectfont
        [CLS] University of Minnesota [SEP] Minneapolis [SEP] \#\#\#  \#\#\#  \#\#\# [SEP] Bloom Island Park [SEP] Bell Museum [SEP] }
    }%
}
\end{center}


% number of neighbors in the dataset (distribution?)
% max token len
\stitle{Training Data}
We constructed a large-scale training set from the OpenStreetMap (OSM) \footnote{OpenStreetMap website: https://www.openstreetmap.org/} %raw 
database of the London and California regions. %The raw OSM data are noisy
To filter out noise in the raw data, we removed entries for entities that missed place names or geo-coordinates attributes. We also discard the entities if the name is not alpha-numeric. 
We randomly choose geo-entities as the pivot and construct the spatial context input as described in \Cref{sec:spatial_context}. 
When searching for the neighbors of a pivot, instead of calculating the distance from the pivot to all the records, we apply the geohashing algorithm \cite{morton1966computergeohash} to prune the majority of records that are far away and definitely out of range (Details in Appendix). The processed dataset contains 69,168 samples in the London area and 148,811 samples in the California area. We use all of them when pretraining \modelname with MLM and MEP. 




\subsection{Inference}\label{sec:inference}
The pretrained \modelname can be used for inference with the geo-entity representation. The direct output of \modelname is the token-level representations. To get entity-level representation $E^p$, we average the token embeddings belong to the $p$ with $E^p = AVG(E^p_1, ...,E^p_t )$, where  $t$ is the length of the tokenized geo-entity\footnote{The pivot entity token length need to be recorded during tokenization}. The geo-entity representation can be used for various downstream applications, including contextualized geo-entity classification and similarity-based inference tasks such as geo-entity typing and geo-entity linking. 

\stitle{Contextualized Classification} is the process of inferring the class types of geo-entities with the contextualized representation. In this paper, we use semantic typing as an example application in this category and try to predict the semantic type (e.g., transportation and healthcare). The problem can be approached as a supervised classification task.
To tackle the task, the final-layer hidden states of the corresponding tokens can be averaged to represent the geo-entity, on top of which a softmax prediction head can be stacked to perform the classification.
%We append a shallow classifier with two fully connected layers to the entity-level feature extraction layer, then fine-tune the model end-to-end with the cross-entropy loss. 

\stitle{Similarity-based Inference} Some tasks involve finding the nearest neighbor in the embedding space. One example is linking the geo-entities in geographical datasets to knowledge bases (KBs), which we refer to as geo-entity linking in this work. %We use WikiData as the target KB in the experiments and treat geo-entity linking as an unsupervised problem. Given the spatial context, we extract entity features for both the query and KB side, then sort the candidates based on the cosine similarity. 
In such a task, contextualized representation of entities can be generated in the same way as that for contextualized classification, based on which the embedding similarity can be directly calculated based on metrics such as cosine distance.

